BenchIE: A Framework for Multi-Faceted Fact-Based Open Information Extraction Evaluation

Intrinsic evaluations of OIE systems are carried out either manually -- with human evaluators judging the correctness of extractions -- or automatically, on standardized benchmarks. The latter, while much more cost-effective, is less reliable, primarily because of the incompleteness of the existing OIE benchmarks: the ground truth extractions do not include all acceptable variants of the same fact, leading to unreliable assessment of the models' performance. Moreover, the existing OIE benchmarks are available for English only. In this work, we introduce BenchIE: a benchmark and evaluation framework for comprehensive evaluation of OIE systems for English, Chinese, and German. In contrast to existing OIE benchmarks, BenchIE is fact-based, i.e., it takes into account informational equivalence of extractions: our gold standard consists of fact synsets, clusters in which we exhaustively list all acceptable surface forms of the same fact. Moreover, having in mind common downstream applications for OIE, we make BenchIE multi-faceted; i.e., we create benchmark variants that focus on different facets of OIE evaluation, e.g., compactness or minimality of extractions. We benchmark several state-of-the-art OIE systems using BenchIE and demonstrate that these systems are significantly less effective than indicated by existing OIE benchmarks. We make BenchIE (data and evaluation code) publicly available on https://github.com/gkiril/benchie.

==> benchie_overview.tex <==
\section{Benchmark overview}

\todo{Basically, explain Fig.~\ref{fig:overview}.}

\begin{figure}[h]
    \centering
    \includegraphics[width=8cm]{benchie-overview2.png}
    \caption{BenchIE overview}
    \label{fig:overview}
\end{figure}

==> old/1-intro-old.tex <==
\section{Introduction (Original Intro)}



%Open Information Extraction (OIE) is the task of extracting relations and their corresponding arguments from natural language text, typically in an unsupervised manner \cite{banko2007open}.
Open Information Extraction (OIE) is the task of extracting relations and their arguments from natural language text in a schema-free manner \cite{banko2007open}. For example, an OIE system is expected to extract the triples \emph{("Sen.~Mitchell"; "is from"; "Maine")} 
and \emph{("Sen.~Mitchell"; "is"; "a lawyer")} from the sentence  \emph{"Sen.~Mitchell, who is from Maine, is a lawyer."}.
%%%
OIE systems are used in many downstream tasks, including knowledge base population \cite{lin2020kbpearl,gashteovski2020aligning}, open link prediction 
\cite{broscheit2020}, and question answering \cite{yan2018assertion}. These downstream tasks lend themselves as natural setups for extrinsic OIE evaluation \cite{mausam2016open}. %w.r.t.~a 
%by measuring the performance on a specific downstream task .
While valuable in concrete applications, such extrinsic evaluations do not measure the intrinsic correctness of the extracted facts: to that effect, several benchmarks for intrinsic OIE evaluation have been proposed \cite{Stanovsky2016EMNLP,lechelle2019wire57,bhardwaj2019carb}.  
%
%OIE system that are not dependent on any particular downstream task. 
%To avoid such dependence on a particular downstream task, OIE systems
%are evaluated intrinsically \cite{mausam2012open,Gashteovski2019OPIECAO,kolluru2020openie6,kolluru2020imojie}.

Automated benchmark evaluations are obviously more feasible (i.e., faster and cheaper) than manual OIE evaluations 
\cite{hohenecker2020systematic}. However, the current benchmarks with scoring functions based on approximate (token-level) matching of system extractions against ground truth facts seem to be substantially less reliable than human judgments of extraction correctness \cite{zhan2020span}.    
%Manual evaluations are usually of higher quality \cite{}, though 
%testing and developing OIE systems with such evaluations is slow, expensive and time-consuming. 
%Such evaluations are usually performed 
%by:~(1) taking a random sample of a number of sentences from a corpus (e.g., Wikipedia);~(2) run OIE systems on them;
%~(3) an expert labeler determines the correctness of each extraction;~(4) compute precision/recall.
%
%Other approach for intrinsic evaluation is with the use of benchmarks \cite{stanovsky2018supervised,hohenecker2020systematic}. 
%In contrast, using benchmarks  is more efficient. \cl{note} %From "In the first attempt" on this is very close to related work, so this is a proposal to save some space.
%In the first attempt for an OIE benchmark, \citet{Stanovsky2016EMNLP} used a dataset from relatively similar task---QA-SRL 
%\cite{he2015question}---and automatically ported it to OIE. Due to the automatic porting, however, the benchmark contains noisy 
%extractions \cite{bhardwaj2019carb}, which in part required human intervention by relabelling the data \cite{zhan2020span}.
%The benchmark CaRB \cite{bhardwaj2019carb} tackles this issue by sampling from the same input sentences %
%\cl{note: same as in the same sentence as for the QA-SRL benchmark?} 
%and relabeling them manually with the use of crowdsourcing. 
%extractions \cite{bhardwaj2019carb}, which sometimes requires human intervention by relabelling the data \cite{zhan2020span}. 
%Both manual and benchmark approaches for evaluation of OIE systems do not consider the problem of incompleteness. In particular, 
%Current benchmarks, however, do not consider the problem of incompleteness. In particular, 
This primarily stems from the \textit{incompleteness} of existing OIE benchmarks: the gold standard extractions do not include \textit{all} acceptable surface realizations of the \textit{same fact}. Consider, for example, a sentence from the recent evaluation framework CaRB \cite{bhardwaj2019carb}: \textit{``Sen.~Mitchell is confident he has sufficient votes to block such a measure with procedural actions''}; with the gold triple extraction (\textit{``Sen.~Mitchell''}; \textit{``is confident he has''}; \textit{``sufficient votes to \dots procedural actions''}). 
%

\begin{table*}
    \centering
    \small
    %\begin{adjustbox}%{max width=\textwidth}
        \begin{tabular}{rrlccc}  
            \toprule
            %& \multicolumn{3}{l}{Input sentence:} \\ 
            \multicolumn{6}{l}{\textbf{Input sentence:} \emph{"Sen.~Mitchell is confident he has sufficient votes to block such a measure with procedural actions."}} \\
            %\multicolumn{3}{l}{\emph{to block such a measure with procedural actions."}} \\
            \multicolumn{6}{l}{\textbf{CaRB golden extraction:} \emph{("Sen.~Mitchell"; "is confident he has"; "sufficient votes to block ...procedural actions")}} \\
            \cmidrule(r){1-6}
            & \multicolumn{2}{c}{Input OIE extraction}    & \multicolumn{2}{c}{CaRB (P / R)} & BenchIE \\
            $t_1$ & \emph{("Sen.~Mitchell"; "is confident he has";} & \emph{ "sufficient")} & 1.00 & 0.44 & 0 \\ 
            $t_2$ & \emph{("Sen.~Mitchell"; "is confident he has";} & \emph{ "sufficient actions")} & 1.00 & 0.50 & 0 \\
            $t_3$ & \emph{("Sen.~Mitchell"; "is confident he has";} & \emph{ "sufficient procedural actions")} & 1.00 & 0.56 & 0 \\
            $t_4$ & \emph{("Sen.~Mitchell"; "is confident he has";} & \emph{ "measure with procedural actions")} & 1.00 & 0.63 & 0 \\
            \cmidrule(r){1-6}
            $t_5$ & \emph{("Sen.~Mitchell"; "is confident he has";} & \emph{ "sufficient votes")} & 1.00 & 0.50 & 1 \\ 
            %$t_5$ & \emph{("he"; "is confident he has";} & \emph{"sufficient votes")} & 0.86 & 0.38 & 1 \\
            \bottomrule
        \end{tabular}
    %\end{adjustbox}
    
    \caption{Difference in scores between CaRB and BenchIE. For the input sentence, CaRB provides only one extraction which covers all the words in the sentence. 
    Then, for each input OIE extraction (from $t_1$ to $t_5$) it calculates token-wise precision and recall scores w.r.t.~the golden annotation. In contrast, 
    BenchIE provides 46 triples for the same input sentence and matches the input OIE extractions with crisp 1/0 scores.} 
    %: \cl{note: add here the conclusion a reader should draw from looking at this}}
    \label{tab:carb-benchie-extractions2}
\end{table*}

Intuitively, a system extraction with a more concise object---(\textit{``Sen.~Mitchell''}; \textit{``is confident he has''}; \textit{``sufficient votes''})---could also be accepted, as it still captures the same core piece of knowledge, and would arguably be valuable in most downstream tasks. 
%), although it does not exactly match the gold extraction.
To account for this, existing benchmarks credit system extractions for per-slot lexical overlap with gold extractions. For example, CaRB \cite{bhardwaj2019carb} aggregates per-slot token-level precision and recall scores between system and gold extractions across the three slots (subject, predicate, and object). Being crowdsourced, CaRB improves over previous benchmarks \cite{Stanovsky2016EMNLP,lechelle2019wire57} by allowing for multiple surface extractions of the same facts. Nonetheless, its scoring based on token overlaps is overly lenient and overestimates the systems' ability to extract correct \textit{knowledge facts}. Consider, e.g., a system extraction (\textit{``Sen. Mitchell''}; \textit{``is confident he has''}; \textit{``procedural actions''}) for the above-mentioned sentence. From the \textit{factual} perspective, this extraction is clearly incorrect  (\textit{Sen.~Mitchell} has \textit{votes}, not \textit{actions}). However, CaRB would judge the extraction as having (1) perfect precision, as all extracted tokens can be found in corresponding slots of a gold extraction and (2) high recall, as all of the gold subject and predicate tokens as well as two gold object tokens (\textit{``procedural''} and \textit{``actions''}) are found within corresponding slots of the system extraction (Table \ref{tab:carb-benchie-extractions2}). 



In this work, we depart from such unreliable and error-prone OIE evaluation based on token matching. We propose BenchIE, a novel \textit{fact-centric} OIE evaluation paradigm at the center of which is the following question: \textit{does the system extraction express the same fact (i.e., the same unit of knowledge) as any of the gold extractions (and vice versa)?} To reliably answer this question, our benchmark exhaustively lists all correct extractions of the same fact. BenchIE specifies \textit{complete} sets of fact-equivalent extractions, which we dub \textit{fact synsets}. We annotate fact synsets for 300 English, Chinese and German sentences, and comparatively evaluate six OIE systems using our new fact-centered evaluation paradigm. BenchIE portrays fact extraction abilities of state-of-the-art OIE models much less favorably and points to their limitations that are not detectable with existing benchmarks.      

% we banchmark ...

%All proposed benchmarks attempt at approximating recall by relaxing the matching protocol for minimizing incidence of false negatives, 
%i.e., correct extractions marked as incorrect. It is not clear, however, how close such approximations are to the true recall and it is highly likely that such 
%benchmarks are perhaps over estimating the recall by being excessively lenient.


%BenchIE addresses this problem by creating a high quality manually annotated dataset that contains all possible variations of the gold extraction for verb mediated relations. This allows us to measure the true recall by directly evaluating the extractions. Therefore, unlike other benchmarks BenchIE does not have to overcompensate for false negatives. By measuring the true recall, BenchIE also measures the quality of approximations of earlier benchmarks. In contrast to previous benchmarks, BenchIE is multilingual, a key feature, that can spur development of multilingual OIE systems. 

%In this paper, we propose BenchIE: a benchmark for intrinsic evaluation of OIE systems. Contrary to previous benchmarks, BenchIE:~
%(1) was constructed with completeness of extractions in mind, which provides more realistic measure of recall; (2) other than English, contains 
%complete extractions in Chinese. Our experiments suggest that current OIE systems have much lower recall and $F_1$ score than previously reported. 
%We propose an evaluation as the level of facts, not at token-overlap levels! To achieve this, it is crucial to annotate all acceptable variants of extractions for the same fact, We call this fact synset. 

%It builds  upon \cite{lechelle2019wire57} by matching the tuples from an extraction with tuples from \textit{multiple} gold extractions, because an extraction can potentially  match other extractions similar to the gold extraction. This is an approximation of the true recall which can only be known if all possible variations of the gold extraction are available and this is essentially the crux of the problem. An extraction can be correct, even when it does not match the correct extractions,  because the set of correct extractions may not be exhaustive enough to cover different variations of the gold extraction.   




%\textit{exhaustively}


%But current benchmarks do not consider the problem of incompleteness. In particular, 
%they do not take into account \emph{all} possible variations of the same fact that can be made from an input sentence. 
%Therefore, they assign token-level precision and recall scores on each extraction. 
%This can be problematic, because even for incorrect extractions, such benchmarks can give overly-optimistic scores
%(see example in Tab.~\ref{tab:carb-benchie-extractions2}). \cl{note} %directly spell out the exhaustiveness and synset contribution, maybe by using the updated example as we discussed in the sync meeting?

%\cl{note: why is this important? maybe also provide an example, what is the danger if a benchmark is used that is not exhaustive?} 
%To address this issue, one  
%approach is to compute the number of correct extractions as a proxy for recall \cite{gashteovski2017minie}, another is to 
%collect all correct extractions produced by all OIE systems as all the possible extractions.\cl{note: what is the issue with these approaches?} As for the benchmarks, they 
%assume that all possible extractions are done 
%\cl{note: this sounds as if benchmarks are exhaustive, what is the difference to "all possible extractions"?}. 
%Because they are not constructed with exhaustiveness in mind, they miss out 
%many extractions that could have been considered, which leads to results that are overly-optimistic w.r.t.~recall and F1 score.
%\cl{note (Bhushan): I have added a few %words on need for exhaustiveness in related works, this paragraph I guess should be merged with related work.}

%In this paper, we propose BenchIE: a benchmark for intrinsic evaluation of OIE systems. Contrary to previous benchmarks, BenchIE:~
%(1) was constructed with completeness of extractions in mind, which provides more realistic measure of recall; (2) other than English, contains 
%complete extractions in Chinese. Our experiments suggest that current OIE systems have 
%much lower recall and $F_1$ score than previously reported. 

%\cl{note}% before the paragraph "Intrinsic evaluations..", I would define what precision and recall mean for OIE, what exhaustivness means in this context and how it is important to measure recall based on an exhaustive annotation. The QA-SRL and Carb description could also be moved to related work (if you need a shorter intro). You could just generally say that manual evaluation and previous benchmarks are not exhaustive, therefore they cannot measure recall.

%\todo{test}

==> old/old-rw.tex <==
\section{Related work}
There are three notable previous OIE benchmarks.
%Indeed \cite{lechelle2019wire57} show that a toy token extraction system can obtain impressive results on OIE2016.
%LONG VERSION
%With the first OIE benchmark, OIE2016, \citet{Stanovsky2016EMNLP} generated an OIE test set by applying a rule based system on a QA-SRL dataset. 
%Due to the automated processing, however, the resulting benchmark contains noise \cite{bhardwaj2019carb}. Additionally, the evaluation protocol also fails to 
%penalize unnecessarily long extractions and does not punish misplacing parts of the predicate with the object and vice versa \cite{lechelle2019wire57}. 
%Consequently, \citet{stanovsky2016getting} updated the matching to \textit{lexical match}, where more than half of the tokens should match the 
%gold triple for the extracted triple to be considered correct.  
%SHORTENED
First, OIE2016 \cite{Stanovsky2016EMNLP} was created by applying a rule based system on a QA-SRL dataset and therefore the dataset is very noisy \cite{bhardwaj2019carb}.  \cl{note:}%this is shortened, long version see above
%RelVis \cite{schneider2017relvis} aims to improve over OIE2016. It contains a dataset composed of OIE2016 along with three other OIE datasets. 
%RelVis modified the OIE2016 evaluation protocol, however it also does not punish overly long extractions due to its containment match of marking an extraction 
%correct if an extraction contains at least one gold standard annotation. Additionally, due to inclusion of OIE2016, it too suffers from noisy gold extractions.
%\citet{zhan2020span} tackled OIE2016's noisy extraction by relabeling the dataset. The evaluation procedure, however, was the same as OIE2016. 
%LONG VERSION
%Wire57 \cite{lechelle2019wire57} introduced a manually annotated high quality OIE test set. They proposed a new procedure for matching extractions 
%based on tuple matching which improves upon OIE2016 by penalising overly long extractions. However, Wire57 only contains 57 test sentences which are not enough 
%for conclusive evaluation. Moreover, the sentences are sampled from a different corpus, which makes it hard to compare it with other benchmarks.
%SHORTENED
Second, Wire57 \cite{lechelle2019wire57} improved upon OIE2016 by using a better tuple matching approach which penalises overly long extractions. However, Wire57 is too small for a conclusive evaluation (57 sentences). \cl{note:}%this is shortened, long version see above

%CaRB \cite{bhardwaj2019carb} introduced a new crowd-sourced dataset for OIE evaluation with around 1200 sentences (down-sampled from OIE2016) and builds 
Third and most recently, CaRB \cite{bhardwaj2019carb} introduced a new crowd-sourced dataset for OIE evaluation with around 1200 sentences (down-sampled from OIE2016). It builds 
upon \cite{lechelle2019wire57} by matching the tuples from an extraction with tuples from \textit{multiple} gold extractions, because an extraction can potentially 
match other extractions similar to the gold extraction. This is an approximation of the true recall which can only be known if all possible variations of the gold extraction are available and this is essentially the crux of the problem. An extraction can be correct, even when it does not match the correct extractions, 
because the set of correct extractions may not be exhaustive enough to cover different variations of the gold extraction. 

All proposed benchmarks attempt at approximating recall by relaxing the matching protocol for minimizing incidence of false negatives, 
i.e., correct extractions marked as incorrect. It is not clear, however, how close such approximations are to the true recall and it is highly likely that such 
benchmarks are perhaps over estimating the recall by being excessively lenient.


BenchIE addresses this problem by creating a high quality manually annotated dataset that contains all possible variations of the gold extraction for verb mediated relations. This allows us to measure the true recall by directly evaluating the extractions. Therefore, unlike other benchmarks BenchIE does not have to overcompensate for false negatives. By measuring the true recall, BenchIE also measures the quality of approximations of earlier benchmarks. In contrast to previous benchmarks, BenchIE is multilingual, a key feature, that can spur development of multilingual OIE systems.    





